Set-Theoretic Types for Polymorphic Variants

Polymorphic variants are a useful feature of the OCaml language whose current definition and implementation rely on kinding constraints to simulate a subtyping relation via unification. This yields an awkward formalization and results in a type system whose behaviour is in some cases unintuitive and/or unduly restrictive. In this work, we present an alternative formalization of poly-morphic variants, based on set-theoretic types and subtyping, that yields a cleaner and more streamlined system. Our formalization is more expressive than the current one (it types more programs while preserving type safety), it can internalize some meta-theoretic properties, and it removes some pathological cases of the current implementation resulting in a more intuitive and, thus, predictable type system. More generally, this work shows how to add full-fledged union types to functional languages of the ML family that usually rely on the Hindley-Milner type system. As an aside, our system also improves the theory of semantic subtyping, notably by proving completeness for the type reconstruction algorithm.

==> intro1.tex <==

Polymorphic variants are a useful feature of OCaml, as they balance
static safety and code reuse capabilities with a remarkable
conciseness. They offer a more flexible alternative to the ordinary
variant types (or algebraic sum data types) of languages of the ML
family. Essentially, ordinary variant types offer a limited form of union
types composed by a finite enumeration of tagged values, with the
caveat that distinct unions cannot share common values; polymorphic
variants add a sort of subtyping and sharing whereby different
variant types may share common values, like classic unions do.

In OCaml, polymorphic variants are typed using a form of parametric
polymorphism called \emph{structural
polymorphism} \cite{Garrigue2002}, which superimposes a system of
kinding constraints over the Hindley-Milner (HM) type system. This is used,
in a sense, to simulate subtyping without actually introducing it in
the system. In general, the current system reuses the ML type
system---including unification for type reconstruction---as much as possible.

We argue that using a different system, one that departs
drastically from HM, is advantageous. In this work we advocate the
use of full-fledged union types with standard set-theoretic subtyping. In particular we
use \emph{semantic subtyping}~\cite{Frisch2008}, a type system where
$(i)$~types are interpreted as set of values, $(ii)$~they are enriched with
unrestrained unions, intersections, and negations interpreted as the
corresponding set-theoretic operations on sets of values, and $(iii)$~subtyping corresponds
to set containment.

In the current system for polymorphic variants,
while kinding constraints are somewhat separated from the rest (which
is why unification and reconstruction can be extended to them), they
still introduce significant complexity and yield a hard-to-grasp formalization of the type system.  Using  set-theoretic types and subtyping
yields a much more natural and easy-to-understand
system in which several key notions---e.g., bounded
quantification and exhaustiveness and redundancy analyses of pattern matching---can be
expressed directly by types; conversely, with structural subtyping they
need meta-theoretic constructions (in the case of kinding) or they are meta-theoretic properties not directly connected to
the type theory (as for exhaustiveness and
redundancy).

The use of structural subtyping not only makes
the theory of polymorphic variants more complicated, but it has several drawbacks in practice as well.
Since its lacks the flexibility offered by a system with true
subtyping, the system may result in unintuitive or overly restrictive behaviour, as shown by the following motivating examples in OCaml.


